RISnet: A Scalable Approach for Reconfigurable Intelligent Surface Optimization with Partial CSI

The reconfigurable intelligent surface (RIS) is a promising technology that enables wireless communication systems to achieve improved performance by intelligently manipulating wireless channels. In this paper, we consider the sum-rate maximization problem in a downlink multi-user multi-input-single-output (MISO) channel via space-division multiple access (SDMA). Two major challenges of this problem are the high dimensionality due to the large number of RIS elements and the difficulty to obtain the full channel state information (CSI), which is assumed known in many algorithms proposed in the literature. Instead, we propose a hybrid machine learning approach using the weighted minimum mean squared error (WMMSE) precoder at the base station (BS) and a dedicated neural network (NN) architecture, RISnet, for RIS configuration. The RISnet has a good scalability to optimize 1296 RIS elements and requires partial CSI of only 16 RIS elements as input. We show it achieves a high performance with low requirement for channel estimation for geometric channel models obtained with ray-tracing simulation. The unsupervised learning lets the RISnet find an optimized RIS configuration by itself. Numerical results show that a trained model configures the RIS with low computational effort, considerably outperforms the baselines, and can work with discrete phase shifts.

==> mmse_precoder.tex <==
\subsection{The WMMSE Precoder}
\label{subsec:precoder}

Unlike the problem of \gls{ris} configuration that is still open,
the \gls{wmmse} precoder is proven to be the optimal precoder to maximize the weighted sum-rate.
It is proved that minimizing \gls{wmmse} is equivalent to maximizing \gls{wsr}~\cite{shi2011iteratively}. 
By iteratively updating precoding vectors and weights of \gls{mse} of each user,
the \gls{wsr} is maximized.
We choose the \gls{wmmse} precoder for the precoding in \gls{bs}.
However, the iterative approach is not differentiable. 
To tackle this problem, we apply \gls{ao}, which updates the precoder matrices $\mathbf{V}$ and phase shift matrices $\mathbf{\Phi}$ alternatively while keeping the other constant for all the data samples.
